GAT: Guided Adversarial Training with Pareto-optimal Auxiliary Tasks

While leveraging additional training data is well established to improve adversarial robustness, it incurs the unavoidable cost of data collection and the heavy computation to train models. To mitigate the costs, we propose Guided Adversarial Training (GAT), a novel adversarial training technique that exploits auxiliary tasks under a limited set of training data. Our approach extends single-task models into multi-task models during the min-max optimization of adversarial training, and drives the loss optimization with a regularization of the gradient curvature across multiple tasks. GAT leverages two types of auxiliary tasks: self-supervised tasks, where the labels are generated automatically, and domain-knowledge tasks, where human experts provide additional labels. Experimentally, GAT increases the robust AUC of CheXpert medical imaging dataset from 50% to 83% and On CIFAR-10, GAT outperforms eight state-of-the-art adversarial training and achieves 56.21% robust accuracy with Resnet-50. Overall, we demonstrate that guided multi-task learning is an actionable and promising avenue to push further the boundaries of model robustness.

==> pages/3-1-results_v2_scarce_data.tex <==


%While all the auxiliary tasks improve the robustness over single-task models, the achieved robustness considerably varies when the strength of the attack is increased. Models adversarially trained with \textbf{Macro} task have their robust accuracy drop by 20\% point while models augmented with the \textbf{Jigsaw} task only show a 0.15\% drop. 

%When comparing the robustness achieved by GAT under PGD-4 and PGD-10 attacks, our results show that some tasks are more robust against stronger attacks. AT with \textbf{Jigsaw} task shows only a 0.15\% drop when we increase the strength of the attack from 4 to 10 iteration attacks.  
%Subsequently, the proper selection of the auxiliary task is critical in limited data scenarios.  

%While there is a 20\% drop of robust accuracy of models augmented with the \textbf{Macro} task when we increase the attack steps from 4 to 10, models augmented with the \textbf{Jigsaw} task only show a 0.15\% drop when the strength of the attack is increased. Subsequently, the selection of the auxiliary task remains a critical question in limited data scenarios.   



%When we compare the improvements obtained on Edema, Atelectasis, and CIFAR-10, our evaluation shows that no one winning auxiliary task outperforms the others for all target tasks.  



\begin{table}[t]
\begin{center}
\small
\caption{Clean and robust accuracy of GAT vs Single task AT for CIFAR-10
models adversarially trained with a 10\% of total data. The values are means and std across 3 runs. % subset of data.
} 
\label{table:cifar10Toy}
\begin{threeparttable}

\begin{tabular}{l||lll}
\hline
            & Test ACC & PGD-10 ACC & PGD-4 ACC \\
         \hline   
Single task & 60.41{\small$\pm$0.62}               & 8.37{\small$\pm$0.32}            & 11.81{\small$\pm$0.20}           \\
\hline
Jigsaw      & 51.98{\small$\pm$0.53}                 & 32.41{\small$\pm$0.46}           & 32.26{\small$\pm$0.22}           \\
\hline
Rotation    & 50.41{\small$\pm$0.11}                & 15.01{\small$\pm$0.29}           &  20.01{\small$\pm$0.15}         \\
\hline
Macro       & 65.62{\small$\pm$0.48}                & 22.42{\small$\pm$0.35}           & 42.68{\small$\pm$0.06}     \\     
\hline
\bottomrule
\end{tabular}
\end{threeparttable}
\end{center}
%\vspace{-3mm}
\end{table}

